A prototype hybrid prediction market for estimating replicability of published work

We present a prototype hybrid prediction market and demonstrate the avenue it represents for meaningful human-AI collaboration. We build on prior work proposing artificial prediction markets as a novel machine-learning algorithm. In an artificial prediction market, trained AI agents buy and sell outcomes of future events. Classification decisions can be framed as outcomes of future events, and accordingly, the price of an asset corresponding to a given classification outcome can be taken as a proxy for the confidence of the system in that decision. By embedding human participants in these markets alongside bot traders, we can bring together insights from both. In this paper, we detail pilot studies with prototype hybrid markets for the prediction of replication study outcomes. We highlight challenges and opportunities, share insights from semi-structured interviews with hybrid market participants, and outline a vision for ongoing and future work.

==> tmkresults.tex <==

Table~\ref{tab:datasummary} provides a summary of the performance of each Hybrid market observation along with its matching fully synthetic market. In all case, the market price reported is the price of the asset that pays \$1 if the paper was declared reproducible in the previous, unannounced, study.\footnote{The market price of the matching non-reproducible asset is always 1 minus the price of this asset by construction.} Thus, we classify a market price as `correct' if it is greater (less) than .5 and the paper was (not) reproducible. The absolute error (AE) is simply the distance between the final price and the value of the asset (0 or 1). Markets with consistently lower AE are considered better predictors. 

To summarize, across the three sessions, the Hybrid Market price is frequently closer to ground truth than the fully synthetic price. The mean AE is .497 in the Hybrid Market versus .552 in the fully synthetic analog; in 9 out of 12 markets the AE is lower in Hybrid Market. A Wilcoxon signed ranks tests fails to reject the null hypothesis that that the distributions of errors between the Hybrid and synthetic markets are the same ($z =-1.373$, $p-value = 1.83$) but this is likely due to the low power of the small sample. In no instance is the Hybrid Market price `not correct' when the synthetic price was `correct' and in one out of 12 instances the Hybrid Market flipped an incorrect prediction of the synthetic market to correct. 

Interestingly, the presence of human traders often induced greater participation by the synthetic agents. In markets 8w97, yDyG and GXEW, no agents participated (conducted trades) in the fully synthetic version resulting in an uniformed price of .5.\footnote{In the absence of trading, the market price for both assets is .5} In three of the four observations involving these markets, the presence of human traders induced agent trades; only in market yDyG with IST researchers were the agents inactive. Further the volume of agent based trades increased from an average of X per market under the fully synthetic condition to Y per market in the Hybrid Market. 

These small sample results indicate that small numbers of informed/expert human traders do not have an obviously deleterious effect on market performance and might even improve accuracy. Likewise, the trading activity of the human traders has the potential benefit of triggering trading by our agent traders. 



\begin{table*}[t]
  \caption{Experimental Data Summary}
  \label{tab:datasummary}
  \begin{tabular}{ccccccccc}
  %\toprule
    Subjects & Market & Ground & Hybrid-M & Hybrid-M & Hybrid-M & AI-M & AI-M & AI-M\\ 
    & & Truth & Final Price & Pred & AE & Final Price & Pred & AE\\ \hline
    %\midrule
Bus & AqDO &    Reproducible & 0.66 &    correct & 0.34 & 0.41 &       Not Correct & 0.59\\
Bus & yDyG &    Reproducible & 0.36 &    Not correct & 0.64 & 0.5 &   No Agent & 0.5\\
Bus & P1rY &    Reproducible & 0.64 &    correct & 0.36 & 0.52 &       correct & 0.48\\
Bus & 8w97 &    Not Reproducible & 0.72 &    Not correct & 0.72 & 0.5 &       No Agent & 0.5\\
IST & AqDO &    Reproducible & 0.38 &    Not correct & 0.62 & 0.41 &       Not Correct & 0.59\\
IST & yDyG &    Reproducible & 0.58 &    correct & 0.42 & 0.5 &       No Agent & 0.5\\
IST & P1rY &    Reproducible & 0.8 &    correct & 0.2 & 0.52 &       correct & 0.48\\
IST & 8w97 &    Not Reproducible & 0.47 &    correct & 0.47 & 0.5 &       No Agent & 0.5\\
Psych & GXEW &    Reproducible & 0.61 &    correct & 0.39 & 0.5 &  No Agent & 0.5\\
Psych &GNjz &    Reproducible & 0.47 &    Not correct & 0.53 & 0.46 & Not correct & 0.54\\
Psych & yypj &    Not Reproducible & 0.76 &    Not correct & 0.76 & 0.86 & Not correct & 0.86\\
Psych & AqDO &    Reproducible & 0.49 &    Not correct & 0.51 & 0.42 &       Not correct & 0.58\\ \hline
%\bottomrule
\end{tabular}
\end{table*}
